er.autopilot 1.0: The Full Autonomous Stack for Oval Racing at High Speeds

The Indy Autonomous Challenge (IAC) brought together for the first time in history nine autonomous racing teams competing at unprecedented speed and in head-to-head scenario, using independently developed software on open-wheel racecars. This paper presents the complete software architecture used by team TII EuroRacing (TII-ER), covering all the modules needed to avoid static obstacles, perform active overtakes and reach speeds above 75 m/s (270 km/h). In addition to the most common modules related to perception, planning, and control, we discuss the approaches used for vehicle dynamics modelling, simulation, telemetry, and safety. Overall results and the performance of each module are described, as well as the lessons learned during the first two events of the competition on oval tracks, where the team placed respectively second and third.

==> tikz/team_exp.tex <==
\begin{tikzpicture}[scale=0.5]
\pie[/tikz/every pin/.style={align=center},
text=pin,
explode=0.2,
sum = auto]{1/PhD \\Students, 3/PostDoc, 11/Master \\Students,  3/Other \\positions}

\end{tikzpicture}


==> tikz/team_field.tex <==
\begin{tikzpicture}[scale=0.5]
\pie[/tikz/every pin/.style={align=center},
text=pin,
explode=0.2,
sum = auto]{6/Computer \\Science , 1/Computer \\Engineering, 3/Robotics \\Engineering, 4/Vehicle \\Engineering,  4/Control \\Engineering}

\end{tikzpicture}

